Review of strongly-coupled composite dark matter models and lattice simulations

We review models of new physics in which dark matter arises as a composite bound state from a confining strongly-coupled non-Abelian gauge theory. We discuss several qualitatively distinct classes of composite candidates, including dark mesons, dark baryons, and dark glueballs. We highlight some of the promising strategies for direct detection, especially through dark moments, using the symmetries and properties of the composite description to identify the operators that dominate the interactions of dark matter with matter, as well as dark matter self-interactions. We briefly discuss the implications of these theories at colliders, especially the (potentially novel) phenomenology of dark mesons in various regimes of the models. Throughout the review, we highlight the use of lattice calculations in the study of these strongly-coupled theories, to obtain precise quantitative predictions and new insights into the dynamics.

==> inputs/sec3-direct.tex <==

Direct detection experiments have long since ruled out dark matter with spin-independent elastic scattering through an electroweak-strength tree-level coupling to the $Z$ boson.  However, the standard model gauge bosons are not ruled out as mediators for standard model-dark matter scattering if their couplings are suppressed.  In composite dark matter models, the occurrence of this suppression naturally occurs through form factors $F(q^2)$, where $q^\mu$ is the momentum transfer through the interaction vertex.  A form factor can be thought of as a momentum-dependent coupling between a force carrier and a composite particle; at $q^2 = 0$ the form factor is equal to the net charge of the composite, while at large $q^2$ it probes the internal constituents.

The interaction of dark matter with ordinary matter mediated by a standard model force carrier can give a distinctive scaling of the interaction cross-section with the choice of nuclear target, depending on the exact nature of the interaction.  A strongly distinguishable case would be photon exchange coupling to the nuclear magnetic moment, which can give a direct detection cross section varying by several orders of magnitude among commonly-used target elements.  More complete effective field theory treatments of how a general dark matter particle can interact with nuclear direct-detection targets have been considered in the literature \cite{Fan:2010gt,Fitzpatrick:2012ix,Cirigliano:2012pq,Hill:2014yka,Hill:2014yxa,Dent:2015zpa}.  For very light (sub-GeV) dark matter, which can arise from some composite models, scattering off of electrons can provide stronger direct-detection bounds \cite{Essig:2011nj,Graham:2012su,Essig:2015cda,Hochberg:2015pha,Hochberg:2015fth} 

We will focus in this review on photon and Higgs-mediated direct detection through moments of the dark matter.  $Z$-boson exchange proceeds through dark moments similar to those for photon exchange, but is additionally suppressed by the $Z$ mass.  Gluon-based interactions are an interesting possibility which have been considered in the literature \cite{Chivukula:1992pn,Godbole:2015gma,Bai:2015swa}.

\subsection{Photon interactions}

If the composite dark matter candidate $\chi$ is neutral, but its constituents carry electromagnetic charge, then its coupling to the photon is proportional to the matrix element
%
\beq
\langle \chi(p') | j_{\rm EM}^\mu | \chi(p) \rangle = F(q^2) q^\mu,
\eeq
%
where $q_\mu = p_\mu + p'_\mu$, $j_{\rm EM}^\mu$ is the electromagnetic current, and $F(0) = 0$.  In the limit that the momentum transfer $|q|$ is very small compared to the compositeness scale $\Lambda$, which is appropriate for dark matter direct detection, the form factor can be described in terms of effective field theory operators of increasing dimension.  The leading C and P-conserving operators are \cite{Bagnasco:1993st,Pospelov:2000bq} the magnetic moment
%
\beq
\mathcal{L} \supset \frac{1}{\Lambda} \bar{\chi} \sigma^{\mu \nu} \chi F_{\mu \nu},
\eeq
%
the charge radius
%
\beq
\mathcal{L} \supset \frac{1}{\Lambda^2} \bar{\chi} \gamma^\nu  \chi \partial^\mu F_{\mu \nu},\ \ \frac{1}{\Lambda^2} \phi^\dagger \phi v^\nu \partial^\mu F_{\mu \nu},
\eeq
%
and the electromagnetic polarizability
%
\beq
\mathcal{L} \supset \frac{1}{\Lambda^3} \bar{\chi} \chi F_{\mu \nu} F^{\mu \nu},\ \ \frac{1}{\Lambda^3} \phi^\dagger \phi F_{\mu \nu} F^{\mu \nu},
\eeq
%
where $\chi$ represents a fermionic dark matter candidate, and $\phi$ a spin-zero bosonic candidate.  If $\phi$ were a boson with non-zero spin, it would also have a magnetic moment operator.  (Note that the dimensions of the operators are the same for scalar dark matter, due to the non-relativistic normalization of the fields which is most appropriate for treating dark matter direct detection \cite{Hill:2014yxa}.)  Other operators at similar orders in the effective expansion, e.g. an electric dipole moment, can appear if CP violation occurs in the dark sector \cite{Pospelov:2000bq}.  Phenomenological treatments of dark matter with some or all of these effective interactions have been considered in the literature, both independently and in the context of composite models \cite{Bagnasco:1993st,Pospelov:2000bq,Sigurdson:2004zp,Gardner:2008yn,Chang:2010en,Banks:2010eh,Barger:2010gv,DelNobile:2012tx,Weiner:2012cb,Pospelov:2013nea,Ovanesyan:2014fha}. 

Detailed formulas for the interaction cross sections mediated by these interactions are derived in the above references.  We will not reproduce them here, but it is worth observing that the scaling of the cross section with the choice of nuclear target can be dramatically different \cite{Dent:2015zpa,DelNobile:2015tza,DelNobile:2015rmp}, depending on which operator dominates.  The per-nucleon interaction cross section is expected to scale as $\mu^2 (J+1)/J$, $Z^2 / A^2$, and $Z^4 / A^{8/3}$ for the magnetic moment, charge radius, and electromagnetic polarizability operators respectively, where $\mu$ is the nuclear magnetic moment, $J$ is the nuclear spin, and $Z$ and $A$ are the standard proton and atomic mass numbers.  (Note that for a dark matter magnetic moment, the scaling given is for the moment-moment interaction; there is also a magnetic moment-nuclear charge interaction \cite{Banks:2010eh,Appelquist:2013ms}, which scales as $Z^2/A^2$ like the charge radius.)

\begin{table}[t]
\begin{tabular}{c|cccc}
\hline
target &	$\mu^2 (J+1)/J$	& $Z^2/A^2$	& $Z^4/A^{8/3}$ \\\hline
Xe 	&1			&1		&1		\\
Si	&0.06681		&1.472	&0.2766	\\
Ge	&0.1130		&1.152	&0.6010	\\
Na	&12.68		&1.357	&0.1798	\\
O	&0.003029	&1.482	&0.1323	\\
I	&17.09		&1.033	&1.018	\\
Ca	&0.004658	&1.476	&0.4464	\\
W	&0.009074	&0.9608	&1.442	\\
Ar	&0.			&1.201	&0.2949	\\
C	&0.02518		&1.481	&0.0900	\\
F	&32.07		&1.331	&0.1341	\\ \hline
\end{tabular}
\label{tab:EM_scaling_normalized}
\caption{Leading scaling of direct-detection interactions involving photon exchange: dark magnetic moment-nuclear moment (first column), dark magnetic moment-nuclear charge or dark charge radius (second column), and dark electromagnetic polarizability (third column), relative to the given prefactor for xenon.  We average over natural isotopic abundance for each element, taking the nuclear magnetic moment $\mu$ and spin $J$ from the literature \cite{Fuller:1976xx}.}
\end{table}
 
The value of these prefactors for several nuclear targets currently used in direct detection experiments are tabulated in Table~\ref{tab:EM_scaling_normalized}, scaled so that the value for xenon is set to 1.  Especially dramatic differences are seen for the coupling to the nuclear magnetic moment.  We also note that the electromagnetic polarizability interaction in principle has a very large uncertainty; since the interaction contains two photons, scattering proceeds through a loop diagram, so this interaction may be particularly sensitive to poorly-known nuclear matrix elements involving excited states \cite{Appelquist:2015zfa}.

On the dark matter side, determination of the coefficients of these operators requires a non-perturbative calculation.  We now turn to lattice calculations focused on photon direct-detection operators.


Calculation of the magnetic moment and charge radius for a given dark matter candidate can be accomplished through a direct lattice calculation of the form factor $F(Q^2)$ itself.  That is, the three-point correlation function
%
\beq
C_3^\mu(t,t') = \sum_{\vec{x}, \vec{y}} e^{-i \vec{p}' \cdot \vec{x}} e^{-i (\vec{p}-\vec{p}') \cdot \vec{y}} \langle B^\dagger(0,0) V^\mu(\vec{x}, t) B(\vec{y}, t') \rangle
\eeq
%
is computed directly, where $B$ is the composite object interpolating operator and $V^\mu$ the electromagnetic current.  Calculating at several values of the discretized momentum transfer and fitting the momentum dependence allows the magnetic moment and charge radius to be determined.

Results on the lattice have been obtained for SU$(2)$ \cite{Hietanen:2013fya} and SU$(3)$ \cite{Appelquist:2013ms} gauge theories.  In the former case, the calculated charge radius for the meson-like dark matter candidate is found to be roughly consistent with its predicted value from vector meson dominance, using the value of the vector-meson mass determined from the lattice as well.  Fairly strong bounds are found from the Xenon100 and LUX experiments, although their model has an additional adjustable parameter $d_b$ which can suppress the charge radius interaction (with $d_b = 0$ corresponding to the restoration of an isospin-like symmetry.)  For the SU$(3)$ study, strong bounds are found particularly from the magnetic moment, restricting the dark matter mass to be larger than roughly 10 TeV from Xenon100 constraints alone. 

Determination of the electromagnetic polarizability can be somewhat more difficult, due to its suppression by large powers of the momentum transfer.  An alternative to direct calculation of the form factor is to apply the background field method \cite{Detmold:2010ts}.  In this approach, a background static electric field $\mathcal{E}$ is applied by use of appropriate boundary conditions in the lattice simulation.  Measuring the ground-state energy of the dark matter candidate as a function of $|\mathcal{E}|$ allows determination of the polarizability from the quadratic Stark shift, e.g.\cite{Appelquist:2015zfa}
%
\beq
E_X(|\mathcal{E}|) = m_X + \left( 2C_F - \frac{\mu_X^2}{8m_X^3} \right) |\mathcal{E}|^2 + \mathcal{O}(|\mathcal{E}|^4), 
\eeq
%
where $C_F$ is the polarizability and $\mu_X$ is the magnetic moment of $X$.

This approach has been used so far to study two different theories on the lattice.  The LSD collaboration has calculated the polarizability in SU$(4)$ gauge theory for their ``stealth dark matter" model \cite{Appelquist:2015zfa}.  In units of the SU$(4)$ baryon mass, the polarizability was found to be comparable to that of the neutron in QCD, much larger than naive dimensional analysis would indicate.  The resulting direct-detection cross section in LUX diminishes rapidly with the dark matter mass and falls below the expected cosmic neutrino background, but an interesting window for direct detection remains below 1 TeV or so.  The polarizability has also been studied in an SU$(2)$ gauge theory \cite{Drach:2015epq} for ``template composite dark matter", finding essentially no bound on their model from direct detection. 

\begin{figure}
\label{fig:pol-su4}
\centering
\includegraphics[width=0.6\textwidth]{figs/Pol_Plot_Corrected_Band}
\caption{Direct detection cross-section prediction for xenon (purple band) for stealth dark matter interacting through electromagnetic polarizability, calculated using lattice results \cite{Appelquist:2015zfa}.  The blue shaded region (top) indicates current experimental bounds from LUX \cite{Akerib:2013tjd}; the grey region (left) shows collider bounds on charged mesons in this model; the orange region (bottom) shows the anticipated irreducible cosmic neutrino background.}
\end{figure}

\subsection{Higgs interaction}

If the composite dark sector contains fundamental fermions $f$, it is natural for them to obtain some of their mass from a Yukawa coupling $y_f$ to the Higgs boson, inducing a mass of order $m_f \sim y_f v$.  If this coupling is present, it will induce a Higgs coupling to any composite state, e.g. a dark baryon $B$ formed from the $f$ fields, of the form
%
\beq
\sum_f y_f \langle B | \bar{f} f | B \rangle.
\eeq
%
This mirrors the way in which the Higgs couplings of the proton and neutron in the standard model arise; they depend on the individual quark Yukawa couplings, and on the scalar-current matrix element, also known as the ``sigma term''.

The coupling to the Higgs need not be the only source of mass for the $f$ fermions; they may also have (technically natural) vector-like mass terms, or Yukawa couplings to other new scalar fields.  In general, we can parameterize the fraction of the fermion mass which is due to the Higgs field by defining the parameter\cite{Appelquist:2014jch}
%
\beq
\alpha = \frac{v}{m_f} \left. \frac{\partial m_f(h)}{\partial v} \right|_{h=v}
\eeq
%
where $m_f(h) = m + yh/\sqrt{2}$, and $m$ encapsulates other sources of mass.  This parameter varies from $\alpha=0$ if $y=0$ (no Higgs contribution to $m_f$), to $\alpha=1$ when $m=0$ (so the Higgs boson is the only source of mass for $f$.)

If the ratio $m_f / m_B$ is kept fixed, then the direct detection cross section for the dark baryon $B$ increases quadratically with $m_B$, leading to fairly strict bounds from current experiments when $\alpha$ is large.  In particular, comparison with LUX yields the bound \cite{Appelquist:2014jch}
%
\beq \label{eq:alpha-bound}
\alpha \lesssim \left( \frac{370\ \rm{GeV}}{m_B} \right)^{1/2} \times \begin{cases}
0.34& m_{PS} / m_V = 0.55, \\
0.05& m_{PS} / m_V = 1,\end{cases}
\eeq
%
where $m_{PS} / m_V$ is the ratio of pseudoscalar to vector meson mass in the SU$(4)$ theory considered, which is a proxy for $m_f / m_B$.  These results strongly disfavor $\alpha = 1$, i.e. a purely electroweak origin for the dark sector fermion masses is essentially ruled out.

Although this result assumes a particular dark sector model based on SU$(4)$ gauge theory, there is some evidence that the constraint $\alpha < 1$ is fairly robust.  The main non-perturbative input which gives the bound Eq.~\ref{eq:alpha-bound} is the ``dark sigma term"
%
\beq
f_f^{(B)} \equiv \frac{\langle B | m_f \bar{f} f | B \rangle}{m_B} = \frac{m_f}{m_B} \frac{\partial m_B}{\partial m_f},
\eeq
%
applying the Feynman-Hellmann theorem to obtain the last equality.  This quantity is readily determined from lattice spectroscopy of the baryon mass vs. input fermion mass.  Lattice results for a number of different gauge theories \cite{DeGrand:2015lna} are shown in Fig.~\ref{fig:sigma-lat}, and indicate that for similar mass ranges, the non-perturbative value of $f_f^{(B)}$ obtained tends to be consistent across different strongly-coupled theories.

\begin{figure}
\label{fig:sigma-lat}
\centering
\includegraphics[width=0.6\textwidth]{figs/sigma-term-lattice}
\caption{Results obtained from lattice simulations\cite{DeGrand:2015lna} in various theories for the ``dark sigma term" $f_f^{(B)}$, defined in the text.  The results are generally quite consistent as a function of fermion mass, even as the gauge group and fermion representation are varied.}
\end{figure}



